The Dynamic Model of the UR10 Robot and its ROS2 Integration

This paper presents the full dynamic model of the UR10 industrial robot. A triple-stage identification approach is adopted to estimate the manipulator's dynamic coefficients. First, linear parameters are computed using a standard linear regression algorithm. Subsequently, nonlinear friction parameters are estimated according to a sigmoidal model. Lastly, motor drive gains are devised to map estimated joint currents to torques. The overall identified model can be used for both control and planning purposes, as the accompanied ROS2 software can be easily reconfigured to account for a generic payload. The estimated robot model is experimentally validated against a set of exciting trajectories and compared to the state-of-the-art model for the same manipulator, achieving higher current prediction accuracy (up to a factor of 4.43) and more precise motor gains. The related software is available at https://codeocean.com/capsule/8515919/tree/v2.

==> Scripts/Figures/comparison-traj-a.tex <==
\begin{figure*}[t]
    \centering
    \newcommand*{\figsize}{0.32\textwidth}

    % Legend
    \begin{center}
    \footnotesize{{\legblue} measured \hspace{0.5em} {\boxgray} nonlinearity region \hspace{0.5em} {\legred} estimated with \cite{gaz_model-based_2018} \hspace{0.5em} {\legyellow} our estimation}
    \end{center}

    % Figure
    \begin{subfigure}[b]{\figsize}
        \centering
        \includegraphics[width=\textwidth]{Images/Plots/Comparison/TrajA/joint1.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{\figsize}
        \centering
        \includegraphics[width=\textwidth]{Images/Plots/Comparison/TrajA/joint2.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{\figsize}
        \centering
        \includegraphics[width=\textwidth]{Images/Plots/Comparison/TrajA/joint3.pdf}
    \end{subfigure}
    \\ \vspace{0.25em}
    \begin{subfigure}[b]{\figsize}
        \centering
        \includegraphics[width=\textwidth]{Images/Plots/Comparison/TrajA/joint4.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{\figsize}
        \centering
        \includegraphics[width=\textwidth]{Images/Plots/Comparison/TrajA/joint5.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{\figsize}
        \centering
        \includegraphics[width=\textwidth]{Images/Plots/Comparison/TrajA/joint6.pdf}
    \end{subfigure}

    % Caption
    \caption{Measured and estimated joint currents in trajectory~A}
    \label{fig:comparison-traj-a}
\end{figure*}


==> Scripts/Figures/comparison-traj-b.tex <==
\begin{figure}[t]
    \centering

    % Legend
    \begin{center}
    \footnotesize{{\legblue} measured \hspace{0.5em} {\boxgray} nonlinearity region \par \hspace{0.5em} {\legred} estimated with \cite{gaz_model-based_2018} \hspace{0.5em} {\legyellow} our estimation}
    \end{center}

    % Figure
    \begin{subfigure}[b]{0.49\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{Images/Plots/Comparison/TrajB/joint1.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{Images/Plots/Comparison/TrajB/joint2.pdf}
    \end{subfigure}
    \\ \vspace{0.25em}
    \begin{subfigure}[b]{0.49\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{Images/Plots/Comparison/TrajB/joint3.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{Images/Plots/Comparison/TrajB/joint4.pdf}
    \end{subfigure}
    \\ \vspace{0.25em}
    \begin{subfigure}[b]{0.49\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{Images/Plots/Comparison/TrajB/joint5.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{Images/Plots/Comparison/TrajB/joint6.pdf}
    \end{subfigure}

    % Caption
    \caption{Measured and estimated joint currents in trajectory~B}
    \label{fig:comparison-traj-b}
\end{figure}

==> Scripts/Figures/uml.tex <==
\begin{figure*}
\centering

\begin{tikzpicture}[font=\tiny]

% Define a UML class named "InverseDynamicsSolver"
\umlabstract{InverseDynamicsSolver}{
    \#inertial\_parameters\_: std::vector$<$double$>$
}{
    +initialize(): void \\
    +\umlvirt{getInertiaMatrix(joint\_positions) : MatrixXd} \\
    +\umlvirt{getCoriolisVector(joint\_positions, joint\_velocities) : VectorXd} \\
    +\umlvirt{getGravityVector(joint\_positions) : VectorXd} \\
    +\umlvirt{getFrictionVector(joint\_velocities) : VectorXd} \\
    +\umlvirt{getTorques(joint\_positions, joint\_velocities, joint\_accelerations) : VectorXd} \\
    +getPayloadMass() : double \\
    +getPayloadCenterOfMass() : std::vector$<$double$>$ \\
    +getPayloadInertia() : std::vector$<$double$>$ \\
    +setPayloadMass(mass: double) : void \\
    +setPayloadCenterOfMass(center\_of\_mass: std::array$<$double, 3$>$) : void \\
    +setPayloadInertia(inertia: std::array$<$double, 6$>$) : void \\
}

% Define a UML class named "Student" that inherits from "Person"
\umlclass[x=10, y=+1]{InverseDynamicsSolverKDL}{
    --chain\_: KDL::Chain \\
    --solver\_: KDL::ChainDynParamPtr
}{
    +initialize(): void \\
}

% Define a UML class named "Teacher" that inherits from "Person"
\umlclass[x=10, y=-2]{InverseDynamicsSolverUR10}{} {
    --getDriveGainsMatrix\_(): MatrixXd
}

% Draw inheritance arrows
\umlinherit{InverseDynamicsSolverKDL}{InverseDynamicsSolver}
\umlinherit{InverseDynamicsSolverUR10}{InverseDynamicsSolver}

\end{tikzpicture}

\caption{IDS' UML class diagram}
\label{fig:uml-diagram}
\end{figure*}


==> Scripts/Tables/comparison-traj-a.tex <==
\begin{table}
\centering
\caption{MSE in \si{\ampere\squared} in trajectory A}
\label{tab:comparison-traj-a}
\begin{tabular}{c|ccc|ccc}
\multirow{2}{*}{\textbf{Joint}} & \multicolumn{3}{c|}{\textbf{estimated with \cite{gaz_model-based_2018}}} & \multicolumn{3}{c}{\textbf{our estimation}} \\
 & $\lvert \dot{\bm q}\rvert > \overline{\dot q}$ & $\lvert \dot{\bm q}\rvert < \overline{\dot q}$ & $\forall \dot{\bm q}$ & $\lvert \dot{\bm q}\rvert > \overline{\dot q}$ & $\lvert \dot{\bm q}\rvert < \overline{\dot q}$ & $\forall \dot{\bm q}$ \\ 
\hline
Joint 1 & 0.7325 & 0.2010 & 0.6221 & 0.0953 & 0.1369 & 0.1039 \\
Joint 2 & 0.4606 & 0.1237 & 0.3579 & 0.1509 & 0.1471 & 0.1498 \\
Joint 3 & 0.1782 & 0.0747 & 0.1625 & 0.0123 & 0.0932 & 0.0246 \\
Joint 4 & 0.0169 & 0.0089 & 0.0156 & 0.0048 & 0.0089 & 0.0055 \\
Joint 5 & 0.0421 & 0.0230 & 0.0377 & 0.0010 & 0.0138 & 0.0040 \\
Joint 6 & 0.0740 & 0.0890 & 0.0776 & 0.0022 & 0.0452 & 0.0126
\end{tabular}
\end{table}

==> Scripts/Tables/comparison-traj-b.tex <==
\begin{table}
\centering
\caption{MSE in \si{\ampere\squared} in trajectory B}
\label{tab:comparison-traj-b}
\begin{tabular}{c|ccc|ccc}
\multirow{2}{*}{\textbf{Joint}} & \multicolumn{3}{c|}{\textbf{estimated with \cite{gaz_model-based_2018}}} & \multicolumn{3}{c}{\textbf{our estimation}} \\
 & $\lvert \dot{\bm q}\rvert > \overline{\dot q}$ & $\lvert \dot{\bm q}\rvert < \overline{\dot q}$ & $\forall \dot{\bm q}$ & $\lvert \dot{\bm q}\rvert > \overline{\dot q}$ & $\lvert \dot{\bm q}\rvert < \overline{\dot q}$ & $\forall \dot{\bm q}$ \\ 
\hline
Joint 1 & 1.5683 & 0.3045 & 1.1878 & 0.1026 & 0.3048 & 0.1635 \\
Joint 2 & 0.4040 & 0.1182 & 0.3357 & 0.2207 & 0.3204 & 0.2446 \\
Joint 3 & 0.1469 & 0.0612 & 0.1330 & 0.0102 & 0.0319 & 0.0137 \\
Joint 4 & 0.0170 & 0.0148 & 0.0168 & 0.0042 & 0.0137 & 0.0052 \\
Joint 5 & 0.0417 & 0.0307 & 0.0375 & 0.0018 & 0.0170 & 0.0075 \\
Joint 6 & 0.0612 & 0.0293 & 0.0563 & 0.0021 & 0.0345 & 0.0071
\end{tabular}
\end{table}
